Predicting Economic Development using Geolocated Wikipedia Articles

Progress on the UN Sustainable Development Goals (SDGs) is hampered by a persistent lack of data regarding key social, environmental, and economic indicators, particularly in developing countries. For example, data on poverty --- the first of seventeen SDGs --- is both spatially sparse and infrequently collected in Sub-Saharan Africa due to the high cost of surveys. Here we propose a novel method for estimating socioeconomic indicators using open-source, geolocated textual information from Wikipedia articles. We demonstrate that modern NLP techniques can be used to predict community-level asset wealth and education outcomes using nearby geolocated Wikipedia articles. When paired with nightlights satellite imagery, our method outperforms all previously published benchmarks for this prediction task, indicating the potential of Wikipedia to inform both research in the social sciences and future policy decisions.

==> 000README.tex <==
nohyperref

==> Poverty Prediction using Remote Sensing Data andText Information(KDD) Arxiv Copy/000README.tex <==
nohyperref

==> Poverty Prediction using Remote Sensing Data andText Information(KDD) Arxiv Copy/00_article_distances.tex <==
\begin{figure}%[h]
    \subfloat[]{
        \centering
        \includegraphics[width=3.35in]{wikipedia_only_model.pdf}
        \label{fig:wikipedia_only_model}
    }
    
    \subfloat[]{
            \centering
            \includegraphics[width=1.6in]{average_distance_to_1_article.png}
            \label{fig:article_distances_1}
    }
    \subfloat[]{
            \centering
            \includegraphics[width=1.6in]{average_distance_to_10_articles.png}
            \label{fig:article_distances_10}
    }
    \caption{\textbf{Top: } The proposed Wikipedia Embedding Model is shown in (a). Our architecture uses textual information to regress on economic development. For a given DHS location, we use the $N$=$10$ closest Wikipedia articles. The blue part is trained on the DHS prediction task, whereas the encoder part of the \textit{Doc2Vec} is pre-trained on the global geolocated Wikipedia article corpus and fixed during training. Panels (b) and (c) show the average distance (km) to the closest and 10th closest Wikipedia articles for each survey location.
    %\s{combine fig 3 and 4, use subfloat}
    }
    \label{Article Distances}
\end{figure}

==> Poverty Prediction using Remote Sensing Data andText Information(KDD) Arxiv Copy/00_ground_truth_dataset.tex <==
\begin{figure*}[t]
    \centering
    \subfloat{
        \includegraphics[width=0.3\textwidth]{wealth-groundtruth-africa.png}
        \label{Ground_truth_africa}}
    \hspace{1.5in}
    \subfloat{\includegraphics[width=0.3\textwidth]{error_range.png}
        \label{Dataset Jitter}}
    \caption{\textbf{Left:} Visualization of ground-truth Asset Wealth Index (AWI) data. Higher values (red) indicate wealthier communities. \textbf{Right:} Jitter in Lagos, Nigeria. Coordinates have up to a 2 km jitter radius in urban areas and 5 km in rural ones.}
    \label{Ground Truth Dataset}
\end{figure*}

==> Poverty Prediction using Remote Sensing Data andText Information(KDD) Arxiv Copy/00_nl_we.tex <==
\begin{figure}[h]
   \subfloat{
        \centering
        \includegraphics[width=1.6in]{ghana_tanzania_NL.png}
   }
   \subfloat{
        \centering
        \includegraphics[width=1.6in]{ghana_tanzania_doc2vec.png}
        }
    \caption{
    %X axes are ground truth, Y axes are predicted wealth.
    Wealth prediction for Nightlight-Only 
    %model 
    (\textbf{Left})  
    %trained on Ghana and tested on Tanzania. Wealth prediction for
    and Wikipedia Embedding (\textbf{Right}) models trained on Ghana and tested on Tanzania.  Nightlights-Only model produces highly correlated results for different ground points, resulting in horizontal lines. Meanwhile, the Wikipedia Embeddings model leads to a better range of predictions.
    %\matthew{Should we explain the horizontal line on the left image?}\chenlin{I guess we can say something about linear correlation and predicted range}\burak{The axis labels and ticks should have larger fontsize.} 
    %\evan{We discuss a plot of the multi-modal results, but we only have 2 plots. Should we include the third plot, or just remove it from our discussion?}\chenlin{we have the third plot, it's just because it is kind of hard to make it look nice when we have 3 plots, so we removed it. If it is necessary, we can add the third one}
    }
    \label{Prediction}
\end{figure}

==> Poverty Prediction using Remote Sensing Data andText Information(KDD) Arxiv Copy/00_number_articles.tex <==
\begin{figure}%[h]
    \centering
    \includegraphics[width=0.350\textwidth]{article_iteration_results.pdf}
    \caption{Pearson's $r^2$ performance for models trained using varying $N$ geographically nearest article embeddings, trained on the specified country and evaluated on Tanzania. 
    %X axis is number of articles, Y axis is Pearson's $r^2$.
    %\s{figure is missing axis labels}
    }
    \label{Article Iteration Graph}
\end{figure}

==> Poverty Prediction using Remote Sensing Data andText Information(KDD) Arxiv Copy/00_pca_analysis.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=2in]{PCA_Analysis.pdf}
\caption{Wikipedia Embedding PCA Analysis. 
The WE model learns to  project the wealthiest $33\%$ quantile to the space closer to \textit{Company}, \textit{Hospital} and \textit{School+University} related Wikipedia Articles' embeddings.} 
%On the other hand, it projects the Top $33\%$ poor predictions to a space further from the articles indicator of wealth.
% \s{takeaway caption}
\label{pca analysis}
\end{figure}

==> Poverty Prediction using Remote Sensing Data andText Information(KDD) Arxiv Copy/00_table_education.tex <==
\begin{table}[h]
\scriptsize
\centering
\begin{tabular}{c c c c c c c c c c c c c c c c c c}
\toprule
& \multicolumn{4}{c}{Trained on} \\
\cmidrule(lr){1-8}
{Tested on} &{Ghana} & {Malawi} &{Nigeria} & {Tanzania} &{Uganda}\\
\cmidrule(lr){1-3}
\cmidrule(lr){3-4}
\cmidrule(lr){4-5}
\cmidrule(lr){5-6}
\cmidrule(lr){6-7}
\cmidrule(lr){7-8}
Ghana &\cellcolor{blue!25} \textbf{0.31} &0.09 &0.11 &0.22 &0.28\\
Malawi &0.21 &\cellcolor{blue!25} \textbf{0.32}  &0.09 &0.23 &0.24\\
Nigeria &0.32 &0.11 &\cellcolor{blue!25} \textbf{0.39} &0.24 &0.23\\
Tanzania &0.27 &0.20 &0.10 &\cellcolor{blue!25} \textbf{0.34} & 0.30\\
Uganda &0.29 &0.19 &0.10 &0.25 &\cellcolor{blue!25} \textbf{0.30}\\
\midrule
Average &0.28 &0.18 &0.16 &0.26 &0.27\\
\bottomrule
\label{table:Education Results Table}
\end{tabular}
\caption{Performances of Wikipedia Embedding model on education level prediction as measured by Pearson's $r^2$. Bolding indicates the best model in each country.}
%--- note that in-country models (shaded) consistently outperform out-of-country models.}
\label{table:Education Results Table}
\end{table}

==> Poverty Prediction using Remote Sensing Data andText Information(KDD) Arxiv Copy/00_table_poverty.tex <==
\begin{table*}[t]
\scriptsize
\centering
\begin{tabular}{l c c c c c c c c c c c c c c c c c c}
\toprule
% & \multicolumn{6}{c}{Pearson's $r^2$ for Wikipedia models} \\
% \cmidrule(lr){2-7}
& \multicolumn{18}{c}{Trained on} \\
\cmidrule(lr){2-19}
& \multicolumn{3}{c}{Ghana} & \multicolumn{3}{c}{Malawi} & \multicolumn{3}{c}{Nigeria} & \multicolumn{3}{c}{Tanzania} & \multicolumn{3}{c}{Uganda} & \multicolumn{3}{c}{All} \\
\cmidrule(lr){2-4}
\cmidrule(lr){5-7}
\cmidrule(lr){8-10}
\cmidrule(lr){11-13}
\cmidrule(lr){14-16}
\cmidrule(lr){17-19}
Tested on & NL & WE & MM & NL & WE & MM & NL & WE & MM & NL & WE & MM & NL & WE & MM & NL & WE & MM \\
\midrule
Ghana & \cellcolor{blue!25} 0.41 & \cellcolor{blue!25} 0.47 & \cellcolor{blue!25} \textbf{0.76} &0.43 &0.42 &\textbf{0.61} &\textbf{0.64} &0.37 &0.45 &0.46 &0.44 &\textbf{0.51} &\textbf{0.65} &0.34 &0.58 &\textbf{0.61} &0.40 & 0.60\\
Malawi &0.30 &0.40 &\textbf{0.48} & \cellcolor{blue!25} 0.24 & \cellcolor{blue!25} 0.49 & \cellcolor{blue!25} \textbf{0.64} &0.34 &0.35 &\textbf{0.55} &0.37 &0.42 &\textbf{0.56} &0.34 &0.25 &\textbf{0.52} &0.40 &0.38 &\textbf{0.56} \\
Nigeria &0.44 &0.32 &\textbf{0.60} &0.31 &0.37 &\textbf{0.52} & \cellcolor{blue!25} 0.30 & \cellcolor{blue!25} 0.52 & \cellcolor{blue!25} \textbf{0.70} &0.46 &0.37 &\textbf{0.57} &0.48 &0.24 &\textbf{0.57} &0.48 &0.35 &\textbf{0.61}\\
Tanzania &0.50 &0.52 &\textbf{0.58} &0.46 &0.52 &\textbf{0.63} &0.52 &0.48 &\textbf{0.64} & \cellcolor{blue!25} 0.60 & \cellcolor{blue!25} 0.64  & \cellcolor{blue!25} \textbf{0.71} &0.52 &0.49 &\textbf{0.63} &0.54 &0.50 &\textbf{0.59}\\
Uganda &0.61 &0.45 &\textbf{0.70} &0.58 &0.50 &\textbf{0.74} &0.62 &0.40 &\textbf{0.70} &0.64 &0.49 &\textbf{0.75} & \cellcolor{blue!25} 0.53 & \cellcolor{blue!25} 0.57 & \cellcolor{blue!25} \textbf{0.76} &0.62 &0.52 &\textbf{0.71} \\
All &0.44 &0.32 &\textbf{0.46} &\textbf{0.55} &0.26 &0.51 &\textbf{0.51} &0.37 &0.48 &0.49 &0.32 &\textbf{0.65} &0.46 &0.27 &\textbf{0.48} & \cellcolor{blue!25} 0.45 & \cellcolor{blue!25} \textbf{0.77} & \cellcolor{blue!25} 0.76 \\
\midrule
Average &0.45 &0.41 &\textbf{0.60} &0.43 &0.43 &\textbf{0.61} &0.49 &0.42 &\textbf{0.59} &0.50 &0.45 &\textbf{0.63} &0.50 &0.36 &\textbf{0.59} &0.52 &0.49 &\textbf{0.64} \\
\bottomrule
\label{table:Results Table}
\end{tabular}
\caption{Performances of Nightlight-Only (NL), Wikipedia Embedding (WE), and Multi-Modal (MM) models on in-country and out-of-country experiments. Columns and rows represent the countries the models were trained and tested on, respectively. The Multi-Modal model outperforms the other models on both in-country (shaded) and cross-country experiments.
}
\label{table:Results Table}
\end{table*}

==> Poverty Prediction using Remote Sensing Data andText Information(KDD) Arxiv Copy/00_wiki_dataset.tex <==
\begin{figure*}%[h]
    % \begin{subfig}
    %     \centering
    %     \includegraphics[width=3in]{diagram/sample_wiki.pdf}
    %     \label{fig:Sample Wiki}
    % \end{subfig}
    % \begin{subfig}
    %     \centering
    %     \includegraphics[width=3in]{diagram/global_wiki.png}
    %     \label{fig:Global Wiki}
    % \end{subfig}
\subfloat{
        \includegraphics[width=0.37\textwidth]{sample_wiki.jpg}
        \label{fig:Sample Wiki}}
\hspace{1in}
\subfloat{
        \centering
        \includegraphics[width=0.37\textwidth]{global_wiki.png}
        \label{fig:Global Wiki}}
    \caption{\textbf{Left:} Example of a geolocated Wikipedia article. Articles such as this contain a wealth of information relevant to economic development. \textbf{Right:} Global distribution of geolocated Wikipedia Articles. Note that there is no overlayed map, and the shape of the continents arises naturally from the spatial distribution of articles.}
    \label{fig:Wiki Dataset}
\end{figure*}

==> Poverty Prediction using Remote Sensing Data andText Information(KDD) Arxiv Copy/00_workflow.tex <==
\begin{figure}%[h]
\centering
\includegraphics[width=3.35in]{workflow.pdf}
\caption{The proposed Multi-Modal architecture. Our architecture uses visual and textual information to regress on survey data. For a given location, we use nightlight imagery and the Wikipedia articles within a certain neighborhood. The blue part is jointly trained on the survey prediction task, whereas the encoder part of \textit{Doc2Vec} is pre-trained on the global geolocated Wikipedia article corpus and kept frozen. 
}
\label{fig:workflow}
\end{figure} 

==> Poverty Prediction using Remote Sensing Data andText Information(KDD) Arxiv Copy/0_abstract.tex <==
Progress on the UN Sustainable Development Goals (SDGs) is hampered by a persistent lack of data regarding key social, environmental, and economic indicators, particularly in developing countries. For example, data on poverty  --- the first of seventeen SDGs --- is both spatially sparse and infrequently collected in Sub-Saharan Africa due to the high cost of surveys. 
Here we propose a novel method for estimating socioeconomic indicators using open-source, geolocated textual information from Wikipedia articles. We demonstrate that modern NLP techniques can be used to predict community-level asset wealth and education outcomes using nearby geolocated Wikipedia articles. When paired with nightlights satellite imagery, our method outperforms all previously published benchmarks for this prediction task, indicating the potential of Wikipedia to inform both research in the social sciences and future policy decisions.

%\s{this is too focused on prior work. the story should be: SDG, important problems, lack of data. here we use wikipedia ..}
%The United Nations' Sustianable Development Goals (SGDs) lay out an important and necessary framework for the global progress of humanity. While these aspirations are of the utmost gravity, often the implementation of programs and the alleviation of problems which work towards the SGDs' achievement are hampered by a persistent lack of data, particularly in certain regions of the globe. This issue is compounded by the inability of local governments to collect the information which the UN and other international organizations rely on for distributing aid and assessing progress towards the SGDs. \matthew{This issue is compounded by high cost of traditional collection methods which prevent local governments from collecting essential information which the UN and other international organizations rely on for distributing aid and assessing progress towards the SGDs.} As such, we propose a novel method for the utilization of open-source textual data, namely Wikipedia, towards socioeconomic ends. We demonstrate our approach by training a neural network to predict the wealth level of spatially fine-grain communities from the latent embeddings of the geolocated Wikipedia articles nearest to them. We then pair this pipeline with the current optimal input for poverty prediction --- nightlights satellite imagery --- and obtain state-of-the-art results for the task. In doing so, we show that Wikipedia, and the latent representations of open-source, geolocated text in general, have the potential to contribute significantly to the prediction of the socioeconomic information required to both assess the SGDs and increase knowledge about regions of the globe that lack the infrastructure to collect local data.

%Poverty prediction has recently gained attention in the machine learning community due to availability of high-resolution inexpensive remote sensing data. For example, with the emergence of such remote sensing data, \cite{Jean790} proposed a transfer-learning driven approach to replace the poverty mapping methods based on the survey data collected in the field which is expensive to obtain. Although usually informative, overhead images can sometimes be not descriptive enough as they tend to look drastically different in different parts of the world. On the other hand, potentially, there exists some other forms of untapped inexpensive data sources that can be complementary to remote sensing data for poverty mapping. In this direction, we explore geo-tagged Wikipedia articles and pair them with the corresponding satellite images to learn multi-modal latent representations. Our experiments indicate that textual representations complement visual representations in poverty mapping as it boosts overall predictive performance in both in-country and out-of-country experiments. Another advantage of textual data is, unlike visual data, it presents low intra-class variance leading to a more general model than the one exploring only visual information for poverty mapping.

==> Poverty Prediction using Remote Sensing Data andText Information(KDD) Arxiv Copy/0_conclusion.tex <==
\section{Conclusion}

In this paper, we propose a novel method for the utilization of geolocated Wikipedia articles for socioeconomic applications. We do this by obtaining vector representations of articles via the $Doc2Vec$ NLP model. We then pair these latent embeddings with survey data and evaluate models to predict poverty and education outcomes: a \wikipedia{} model, and a \multimodal{} model that also uses nightlights information. Using this framework, we find Wikipedia articles to be informative about socioeconomic indicators. To the best of our knowledge, this is the first time Wikipedia is used in this way. Additionally, the \multimodal{} model outperforms current state-of-the-art results for the poverty prediction task by over $20\%$. 
%To better understand these findings, we then train an ablative Nightlights-Only Model to evaluate the effectiveness of the Multi-Modal Model without Wikipedia embedding input. 
Our findings suggest this pipeline, and the geolocated Wikipedia article dataset, has applications not just in poverty analysis, but also more general socioeconomic prediction, such as education and health related outcomes. This novel approach could lead to advances in development economics, where studies often rely only on nightlights information. Additionally, we hope this approach will accelerate progress towards the UN SDGs by improving the way we estimate lacking socioeconomic indicators, particularly in developing countries, with the aim of improving responses from regional governments and international aid organizations.\\

%After continued research in this new, promising space by the AI community, we look forward to the deployment of systems such as this into the field.  for the betterment of society.
%, with specific qualities that allow us to treat it as a proxy for local geographic knowledge, we are able make socioeconomic predictions about the region around them. We use a self-supervised approach to learn a latent representation for Wikipedia articles. 

%We observe that such a process allows for the creation of a model which can be utilized for poverty prediction, and, when combined with the traditional CNN - nightlight approach used for such tasks, sets new state of the art benchmarks for the problem. We believe this novel approach to applied Machine Learning possesses the potential to revolutionize the space, and, after further iterations and additional exploration, we look forward to the deployment of systems such as this into the field for the betterment of society.

%%%%%%%%%%%% Other tasks


\noindent\textbf{Reproducibility:} Upon publication, we will publicly release our Wikipedia, nightlights and processed indexes data. Raw DHS surveys can be obtained from the World Bank, while Afrobarometer is available through AidData.

==> Poverty Prediction using Remote Sensing Data andText Information(KDD) Arxiv Copy/0_datasets.tex <==
\section{Datasets}

In this section, we describe the ground truth data for the indexes used to measure poverty and education as well as the collection of Wikipedia articles and nightlight images.

\input{00_ground_truth_dataset.tex}

%%%%%%%%%

\subsection{Socioeconomic data}
%\marshall{I edited the below and it should be good to go.}
Our ground truth dataset consists of data on asset ownership from the Demographic and Health Surveys (DHS)~\cite{DHS} and Afrobarometer~\cite{AFRO}. DHS is a set of nationally-representative household surveys conducted periodically in most developing countries, spanning 31 African countries. Afrobarometer (Round 6) is a survey across 36 countries in Africa, assessing various aspects of welfare, education, and infrastructure quality.
%, where each of these points corresponds to a real world coordinate $c_{i}$ and possesses a wealth index $y_{i}$. 
While data from the DHS and Afrobarometer has been used as training data in multiple machine learning applications~\cite{Jean790,blumenstock2015predicting,Xie2016TransferLF,Oshri:2018:IQA:3219819.3219924}, it is both costly to create and sparse in its coverage. 
Typically, the door-to-door surveys used in DHS are conducted approximately every five years, resulting in poor temporal resolution. Each survey also yields only a few thousand data points per country, even for nations with tens of millions of residents. This means the data captures only a tiny fraction of the population, often leading to entire regions within countries being left out of the survey. Additionally, these surveys are not conducted in every country, and destabilized and dangerous regions of the globe can be excluded due to the hazard presented to interviewers.

From the available DHS survey data, we compute an Asset Wealth Index (AWI) as the first principal component of survey responses to questions about asset ownership (e.g. ownership of bicycles, cars, etc.); this approach is a common one for building a measure of wealth from survey data ~\cite{filmer1999effect,smits2015international}. To make this index comparable across all our African countries, we compute the PCA on the data pooled across all countries and survey years, yielding a normalized measure scaled between approximately -2 and 2 (see Fig.~\ref{Ground Truth Dataset}). We aggregate household-level AWI estimates to the village level -- the level at which our latitude and longitude data are available -- yielding a training set where labels correspond to a wealth index $y_{i}$ for each lat/lon coordinate $c_{i}$ where the survey was taken. To protect privacy, the recorded coordinate $c_{i}$ for each datapoint provided by DHS contains up to 5 km of added noise in rural areas and 2 km of noise in urban areas. This limits the usable spatial resolution of the data. A visualization of this effect is in Fig.~\ref{Ground Truth Dataset}, right.

To test the effectiveness of our approach on different outcomes, we also use an education index directly from Afrobarometer, capturing the local level of education in a community. The use of Afrobarometer, a survey conducted by a different organization and with a different methodology, allows us to further test the generality of our approach.
%Here, the AWI $y_{i}$ is a measure of total assets/capital held by a household, normalized across Africa and scaled between approximately -2 and 2 (see Fig. \ref{Ground Truth Dataset}).
%\s{justify this. can we refer to prior work using this methodoology? if not, we need to motivate this} 
%\chenlin{be careful about the range here, looks like our actual data can be larger than 2 as shown in the diagram}
%This measure is calculated by recording the number of various items (e.g., bicycles, cars, etc.) and the amount of cash a household possesses. Following standard practice, the weight of different assets is obtained via Principal Component Analysis (PCA)~\cite{filmer1999effect,filmer2012assessing,smits2015international}. 
%\neal{You guys are just using the DHS AWI directly right? If so, just say that it comes directly from the DHS and is computed as the first principal component of survey responses to questions about asset ownership. What does it mean to be normalized across Africa though? Does this mean that you actually constructed this asset index yourself?}

%%%%%%%%%

\subsection{Geolocated Wikipedia Corpus}
%\s{here describe the inputs. do not mention \textit{Doc2Vec} or any methods}
%\evan{need to contrast the coverage/density of the poverty data with that of wikipedia; mention that the interaction between different sets of wikipoints allow inference regarding wealth (so the sparsity of articles isnt a huge issue).}
%\matthew{Should we cite the Wiki dataset paper here? This seems to imply that the dataset was created for this task.}
Our input dataset consists of a corpus of geolocated Wikipedia articles $D$. To obtain it, we parsed the June 2018 Wikipedia article dump into its constituent documents and then extracted all those that were geolocated (i.e., associated with a specific latitude and longitude). This process netted over 1 million geolocated articles globally (see Fig.~\ref{fig:Wiki Dataset} for this distribution as well as an example article). Of note is that throughout Africa there are roughly 50,000 such articles. 
These geolocated articles are about topics encompassing many categories, including infrastructure (i.e., bridges and roads), populated places, companies, and others. While some articles contain structured information in their infoboxes, many simply contain unstructured text data in their article bodies. 
%This has made Wikipedia difficult to use for the social sciences in the past. 
%\matthew{The last sentence is already in the intro}
%, meaning that all the articles in the neighborhood of $c_i$ that are used as inputs to predict $y_i$ come from this subset of the 1.02 million globally.
% We then trained a \textit{Doc2Vec} model \cite{mikolov2013efficient} on the text corpus to learn a feature-rich, latent space representation of the articles in a self-supervised manner. This compresses each article in to a vector in $\mathbb{R}^{300}$.
%%%%%%%%%

\subsection{Nightlights Imagery}

In addition to learning textual features from geolocated Wikipedia articles, we utilize (5 km $\times$ 5 km) nightlights images compiled by \cite{nips_2017_workshop_stefano}. 
These images are composed of high-resolution night-time imagery from VIIRS \cite{VIIRS} and are of shape $(255,255)$. For each point in the AWI data that we train on, we obtain a nightlights image centered on its coordinate $c_i$. The size of these images was set to (5 km $\times$ 5 km) due to the (maximum) 5 km noise that each location $c_i$ has.
Nightlights information has been shown to be highly correlated with economic development~\cite{Xie2016TransferLF}. However, nightlights are less effective in the poorest quantiles of the population~\cite{Jean790}. In fact, there are numerous locations that are completely dark at night, yet exhibit significant variation in terms of wealth index (see Fig.~\ref{Prediction}). This motivates the use of alternative covariates for prediction, such as Wikipedia articles.

%%%%%%%%%
%%%%%%%%%

%In particular, it is highly useful for separating rich region from poor region. By coupling Wikipedia articles to nightlight images we hope to learn dual complementary representations.

%\subsection{Dataset Limitation}
%\evan{Not sure this part is necessary}
%\burak{Yes, it does not seem very necessary. Later, if we have space we can add it.}
% Our image dataset and poverty measurements are from varying years (based on the country surveys). However, our Wikipedia article dataset is built from Wikipedia articles scraped in 2018. As such, we make the assumption that the pairing of 2018 articles with older nightlights imagery is actionable and robust. Moreover, this presents an implicit assumption in our model that the physical structures in these articles have not changed drastically since the dataset's creation, or that the articles remain accurate. However, we note that the structures in these geolocated articles existed with our without the Wikipedia articles, so a Wikipedia-supplemented model should only improve upon the lower bound of poverty models without Wikipedia. Therefore, the newest Wikipedia articles allow the model to gain additional information on the location. We leave gathering the date each article was authored in order to remove this bias to future work. 



==> Poverty Prediction using Remote Sensing Data andText Information(KDD) Arxiv Copy/0_interpretability.tex <==
\subsection{Ablation study and Interpretability}

%\s{can we say that performance generally improves as $N$ grows?
%we might also need to explain why it's not monotonic
%}

%\matthew{It seems like its plateauing as $N$ gets large. }

So far we have presented our results for both architectures using $N=10$ closest articles to the ground truth point. To evaluate the sensitivity to $N$, we conducted additional experiments by varying number of articles $N$. As shown in Fig.~\ref{Article Iteration Graph}, considering average performance, we can conclude that $N=10$ provides good performance for most of the countries.
%\s{remoe egypt, also from figure 7}
However, for some countries (Uganda, Tanzania), even a few articles can provide optimal models. We believe this might be due to the different density of articles (see Fig.~\ref{fig:article_distances_1}, and ~\ref{fig:article_distances_10}) around data points. 
%Considering different densities of articles in different countries, it is not practical to find a country-agnostic value of number of articles.

\input{00_number_articles.tex}
\input{00_pca_analysis.tex}

To help us better understand Wikipedia article embeddings, we performed a PCA analysis of the learned Wikipedia article embeddings. More specifically, we trained a model on Tanzania, evaluated it on Uganda, ranked all its projections from richest to poorest, and then stored the top third and bottom third of these points, corresponding to the richest $33\%$ and the poorest $33\%$ of all projections for Uganda. For each of the points in these wealthiest and poorest thirds, we averaged the embeddings of the 10 closest articles to it. We then compared these averaged embeddings' PCA projections to the projections of `school', `university', `hospital', `company', and `settlement' articles that appeared in the test set (see Fig.~\ref{pca analysis}). We observed that the average \textit{Doc2Vec} embeddings of the wealthier coordinates clustered around article categories which intuitively are related to wealth. In particular, wealthier places tended to cluster toward `school', `university', `hospital', and `company' embeddings, while poorer places were more related to `settlement' articles.

==> Poverty Prediction using Remote Sensing Data andText Information(KDD) Arxiv Copy/0_intro.tex <==
\section{Introduction}

\input{00_wiki_dataset.tex}

The number one goal of the United Nations Sustainable Development Goals is to "end poverty, in all its forms, everywhere." While much has been done to achieve this objective, there still remain vast regions of the world where extreme poverty continues to be a persistent and endemic problem. Progress is hampered by a stubborn lack of data regarding key social, environmental, and economic indicators that would inform research and policy. Many nations lack the governmental, social, physical, and financial capabilities to conduct large-scale data gathering operations and costly on-the-ground surveys to identify and distribute aid to the most needy communities~\cite{sahn2000poverty}.
Unfortunately, this data scarcity is typical of other SDGs as well: healthcare and mortality data \cite{kahn2007research}, infrastructure and transportation statistics, economic well-being and educational achievement information, food security \cite{antwi2012mapping} and wealth inequality assessment, among many others. This lack of detailed and consistent information contributes to delayed or suboptimal financial and physical responses from both regional governments and international aid organizations. 

There have been numerous attempts to remedy this shortage of socioeconomic information through the combination of machine learning with cheap, globally available data streams such as social media or remotely sensed data. 
In particular, with regard to healthcare data, \cite{signorini2011use} use Twitter as an information-rich source from which to track and predict disease levels and the public's concerns regarding pathogens, while \cite{carneiro2009google} pursue a similar task via the analysis of Google trends. \cite{pulse2014mining} mine the tweets of Indonesian citizens in order to understand food shortages as well as analyze food security and predict food prices on a granular level. 
%,and \cite{chen2014mining} utilize Twitter to track and understand %educational achievement and satisfaction. 
\cite{nikfarjam2015pharmacovigilance} also utilize social media posts to track adverse reactions to drugs with the hope of increasing the scale of data available in the healthcare space. Finally, \cite{blumenstock2015predicting} use mobile phone metadata to attempt to predict poverty levels for data-sparse regions of Rwanda, and \cite{xu2016cross} successfully perform detailed traffic prediction using the open-source geospatial dataset OpenStreetMap (OSM) \cite{haklay2008openstreetmap}.

In this paper, we propose the use of Wikipedia as a previously untapped source of data to estimate socioeconomic indicators at very high spatial resolution. Our approach is motivated by both the sheer scale and information-richness of Wikipedia (see Fig. \ref{fig:Wiki Dataset} for a spatial distribution of articles), as well as the ease with which its geospatial nature can be exploited. Indeed, in the English Wikipedia alone, there are over 5.7 million entries, each of which averages 640 words in length. Of these, 1.02 million are geolocated (i.e., associated with a physical coordinate) (Fig. \ref{fig:Wiki Dataset}), allowing them to be used for spatial socioeconomic indicator prediction. Surprisingly, many developing regions of the world contain high concentrations of geolocated articles, with 50,000 for the continent of Africa alone. By providing detailed textual information about locations and entities in an area (e.g., articles about dams, schools, hospitals), we view the articles as data-rich proxies representing the regions around them~ \cite{sheehan2018learning,uzkent2019learning}. In principle, articles like these contain socioeconomic information, though it is often more qualitative than quantitative. Because much of this qualitative data is in unstructured article bodies, and not in infobox/structured formats, it is difficult to extract --- this difficulty has prevented Wikipedia from being integrated fully into social science research.

% this paragraph is not necessary
%Due to an abundance of benchmarks with which to compare our results, as well as the availability of ground truth datasets from Sub-Saharan Africa conducive to machine learning applications, we focus our efforts on predicting economic well-being/poverty using our Wikipedia corpus. Since performing poverty prediction is considered to be a simpler task than conducting health outcome and mortality rate projection, etc., we feel that validating our approach on this problem demonstrates the potential it may have with regard to predicting other socioeconomic metrics as a proof of concept. Finally, many current processes for this task involve heavy overhead and are resource intensive. Indeed, modern state-of-the-art attempts to predict poverty, such as \cite{Jean790} and \cite{nips_2017_workshop_stefano}, rely on the utilization of nighttime "nightlights" satellite imagery, an approach which: 1) requires access to real time, high-resolution, often expensive data unobstructed by cloud cover, 2) uses data differing from one part of the globe to another in terms of its pixel value and geospatial distribution, and 3) possesses significant room for improvement regarding its accuracy in regression predictions.

As such, we propose leveraging recent advances in NLP to extract information from free-text Wikipedia articles. We first map geolocated articles to a  vector representation using the $\textit{Doc2Vec}$ method \cite{le2014distributed}. We then use the spatial distribution of these embeddings to predict socioeconomic indicators of poverty, as measured by ground-truth survey data collected by the World Bank.
Using the latent embeddings of nearby geolocated Wikipedia articles to predict the wealth level of geographic locales, we demonstrate that, on its own, Wikipedia is a strong socioeconomic predictor of poverty across 5 Sub-Saharan African nations: Malawi, Nigeria, Tanzania, Uganda, and Ghana. 
%We achieve Pearson's $r^2$'s of .49, .52, .64, .57, and .47, respectively, as compared to current nightlight state-of-the-art results of .55, .69, .58, and .66 (Ghana not included in previous study). 
%\neal{Is this the quantitative comparison that we want to make? Maybe we should just compare the multi-modal results?}
We further extend our models to incorporate local information about nightime-light intensity as measured by satellites.
We then show that this multi-modal approach combining textual information and remotely sensed data significantly improved state-of-the-art results for the task of poverty/economic well-being prediction across these same 5 countries. We achieve Pearson's $r^2$'s of .64, .70, .71, .76, and .76, respectively, as compared to current nightlight state-of-the-art results of .55, .69, .58, and .66 (Ghana not included in previous study). 
%\neal{Could give the $r^2$ comparisons here... also sounds awkward right now.}
Additionally, our approach is able to provide reliable predictions of education-related outcomes, indicating that it can generalize to different types of socioeconomic indicators. 
We believe the varying data sources and data types in this multi-modal approach provide our models with much more descriptive features. To the best of our knowledge, there has not heretofore been any work done utilizing multi-modal data for poverty prediction.



%%%%%%%%%
%%%%%%%%%


%\s{end saying you focus on predicting economic well-being/poverty}
%Traditional methods of poverty prediction and estimation revolve around the utilization of laborious and expensive on-the-ground surveys. While these surveys are often quite accurate and precise, it is highly impractical and costly to increase their temporal frequency. Additionally, many regions of the globe lack the infrastructure to even conduct them at a reasonable frequency. As such, it is in the best interests of society, as well as institutions such as governments, Non-profits, the UN and World Bank, and private industry, to explore and implement more cost-effective, tractable, and scalable solutions.

%Our contributions are: (1) We extend previous work  \cite{nips_2017_workshop_stefano} \cite{Xie2016TransferLF} with novel data sources and show its effectiveness at predicting poverty, achieving state-of-the-art results in the process. (2) We test the data across national boundaries, ensuring no train-test contamination. (3) We present promising results that are trivially generalizable to other countries outside of Africa. 

%The United Nations Sustainable Development Goals clearly states that the foremost aim of the global community is to "end poverty, in all its forms, everywhere." \cite{UNGoals} While much has been done to achieve this objective, there still remain vast regions of the world where extreme poverty continues to be a persistent and endemic problem. Many nations in these areas lack the governmental, social, and physical financial capabilities to adequately combat such issues, especially given the necessity \s{you might want to make this link more explicit. poverty, sdgs are important. we lack reliable data on many of them. this makes research, policy, etc less effective. } of using large-scale data gathering operations and costly on-the-ground surveys to identify and distribute aid to the most needy communities \cite{sahn2000poverty}. Unfortunately, this shortage of knowledge extends into many other vital arenas, not limited to: healthcare and mortality data \cite{kahn2007research}, infrastructure and transportation statistics, economic well-being and educational achievement information, and crop yield \cite{antwi2012mapping} and wealth inequality assessment, among numerous other things. In many of these countries, the World Bank and other international organizations are the only collectors of this vital life-saving data, contributing to delayed and inadequate financial and physical responses from both the UN and regional governments due to a lack of detailed and consistent information from local authorities. \s{empahsize that surveys are good but costly. done infrequently, cover a small (represetative) sample of a population }

%There have been numerous attempts to remedy this shortage of socioeconomic information through the use of social media and open-source datasets. \s{cheap, passively collected, widely available} In particular, with regard to healthcare data, \cite{signorini2011use} use Twitter as an information rich source from which to track and predict disease levels and the public's concerns regarding pathogens, while \cite{carneiro2009google} pursue a similar task via the analysis of Google trends. \cite{pulse2014mining} mine the tweets of Indonesian citizens in order to understand food shortages as well as analyze food security and predict food prices on a granular level, and \cite{chen2014mining} utilize Twitter to track and understand educational achievement and satisfaction. \cite{nikfarjam2015pharmacovigilance} also utilize social media posts to track adverse reactions to drugs with the hope of increasing the scale of data available in the healthcare space. Finally, \cite{blumenstock2015predicting} use mobile phone metadata to attempt to predict poverty levels for data sparse regions of Rwanda, and \cite{xu2016cross} successfully perform detailed traffic prediction using the open-source geospatial dataset Open Street Map (OSM) \cite{haklay2008openstreetmap}.

%\s{large body of research exploring the use of social media. google flu, rice prices from twitter data, OSM for xxx, etc. cite a few examples. here we explore the use of wikipedia}
%Research into the corpus and distribution of geolocated Wikipedia articles has suggested they could possibly contribute to socioeconomic factor prediction \cite{sheehan2018learning}. 
%\s{discuss the data: coverage, lots of info, etc.}
%In this paper, we explore using Wikipedia towards a similar end, namely, as an open-source, information-rich well of data from which to make socioeconomic factor prediction. Such an approach is motivated by both the sheer scale and textual detail of Wikipedia (Fig. \ref{fig:Wiki Dataset}) as well as by the ease with which its geospatial nature can be exploited. Indeed, in the English Wikipedia alone, there are over 5.7 million entries, each of which averages 640 words in length \cite{Wikistats}. Of these 5.7 million, 1.02 million are geolocated (associated with a physical coordinate) (Fig. \ref{fig:Wiki Dataset}), allowing them to be used for regional socioeconomic prediction. Surprisingly, many developing regions of the world contain concentrations of geolocated articles, with 50,000 for the continent of Africa alone. By providing detailed textual information about locations and entities in an area, we view the articles as data rich proxies representing the region around them. In principle, articles like these contain socioeconomic information, though it is often more qualitative than quantitative. Because much of this qualitative data is in unstructured article bodies, and not in infobox/structured formats like quantitative data, it is difficult to extract. This has prevented Wikipedia from being integrated fully into the social sciences up to this point. As such, though article types are diverse (e.g. dam, town, company) and almost never contain explicit information/statistics on wealth, healthcare, mortality, etc. for the data sparse regions of the world we examine, in aggregate we believe they possess a confluence of latent features which are robust predictors of socioeconomic metrics. 
%\s{explain that suprisingly, there are many articles in developing regions as well. articles contain in principle a lot of information about socio-economic..structured data (e.g. infoboxes) is limited, so most of the useful information is in the text. unstructured data has largely prevented its use in the social sciences. }

% this paragraph is not necessary
%Due to an abundance of benchmarks with which to compare our results, as well as the availability of ground truth datasets from Sub-Saharan Africa conducive to machine learning applications, we focus our efforts on predicting economic well-being/poverty using our Wikipedia corpus. Since performing poverty prediction is considered to be a simpler task than conducting health outcome and mortality rate projection, etc., we feel that validating our approach on this problem demonstrates the potential it may have with regard to predicting other socioeconomic metrics as a proof of concept. Finally, many current processes for this task involve heavy overhead and are resource intensive. Indeed, modern state-of-the-art attempts to predict poverty, such as \cite{Jean790} and \cite{nips_2017_workshop_stefano}, rely on the utilization of nighttime "nightlights" satellite imagery, an approach which: 1) requires access to real time, high-resolution, often expensive data unobstructed by cloud cover, 2) uses data differing from one part of the globe to another in terms of its pixel value and geospatial distribution, and 3) possesses significant room for improvement regarding its accuracy in regression predictions.

%\s{propose to use \textit{Doc2Vec}, show that it works, can be combined with nighlights} 
%As such, we propose a novel method for the utilization Wikipedia as an open-source dataset to both combat the lack of real time local data from many parts of the globe as well as supplement current approaches using nightlights imagery. Using the latent embeddings of nearby geolocated Wikipedia articles to predict the wealth level of geographic locales, we demonstrate that, on its own, Wikipedia is a strong socioeconomic predictor of poverty. This is done on a granular scale across 5 Sub-Saharan African nations that often serve as benchmarks for the task: Ghana, Malawi, Nigeria, Tanzania, and Uganda. We utilize the NLP feature extractor and latent space encoder \textit{Doc2Vec} \cite{mikolov2013distributed} to obtain these embeddings, which are used as input for the model. This approach yields surprisingly successful results, with pearson's $r^2$ ranging from .24 to .77 for our experiments (Table \ref{table:Results Table}). In light of the common practices of the space, we then extend our models to incorporate multi-modal nightlight-article datasets formed of (nightlight image - article embedding) pairings. We then show that this ensembling yields new, significantly improved state-of-the-art results for the task of poverty/economic well-being prediction across these same 5 countries. We believe the varying data sources and data types in this multi-modal approach provide our models with much more descriptive features. To the best of our knowledge, there has not heretofore been any work done utilizing multi-modal data to this extent for poverty prediction. 

%\s{end saying you focus on predicting economic well-being/poverty}
%Traditional methods of poverty prediction and estimation revolve around the utilization of laborious and expensive on-the-ground surveys. While these surveys are often quite accurate and precise, it is highly impractical and costly to increase their temporal frequency. Additionally, many regions of the globe lack the infrastructure to even conduct them at a reasonable frequency. As such, it is in the best interests of society, as well as institutions such as governments, Non-profits, the UN and World Bank, and private industry, to explore and implement more cost-effective, tractable, and scalable solutions.

%Our contributions are: (1) We extend previous work  \cite{nips_2017_workshop_stefano} \cite{Xie2016TransferLF} with novel data sources and show its effectiveness at predicting poverty, achieving state-of-the-art results in the process. (2) We test the data across national boundaries, ensuring no train-test contamination. (3) We present promising results that are trivially generalizable to other countries outside of Africa. 

%%%%%%%%%
%\s{the logic of the intro is good now. you might want to change the wording/style a bit, try to be more ``dry'' and technical. short factual sentences.}

==> Poverty Prediction using Remote Sensing Data andText Information(KDD) Arxiv Copy/0_methods.tex <==
\section{Methods}

%\s{define the task using the notation you introduced before. predicting $y$ using ..}
%\s{explain why is the problem challenging? you are using unstructured data (text)}
We consider the task of predicting the wealth level $y_{i}$ at various locations $c_{i}$ (represented by a latitude, longitude pair) using geolocated Wikipedia articles from a suitable neighborhood of $c_{i}$. In order to accomplish this, we use the AWI data described in the previous section as ground truth to train and evaluate our model.
%\s{actually, our task is to predict $y$ from wikipedia articles. we use the DHS as training and validation data}
Processing these Wikipedia articles poses a large challenge due to the unconstrained textual data they contain. Much of the data is not stored in structured quantitative ``infobox'' format, but instead in qualitative and textual format in the article bodies. 
%This has made Wikipedia somewhat inaccessible to the social sciences up to this point.  
As an example, one can consider the articles on \textit{Kampala}
%\footnote{\url{https://en.wikipedia.org/wiki/Kampala}} 
and \textit{Masaka}
%\footnote{\url{https://en.wikipedia.org/wiki/Masaka}}
, two different cities in Uganda. 
%While both articles contain infoboxes, the data inside them is already accessible to researchers via the sources the article author(s) used and cited. Often, such sources are the UN and local governments, defeating the purpose of extracting this data from Wikipedia in the first place.
%\neal{I don't think I understand the point that these two sentences are trying to make.}
%Yet this information is very sparse. 
In these articles, the infobox data contains only population totals, weather data, elevation, and a few other easily obtained metrics. However, in the unstructured body text, much richer qualitative data is available. For instance, the Kampala article describes construction of a new light rail system in the city, as well as efforts to relocate heavy industry to ease traffic. 
%\matthew{Is there an example in the article more obviously linked to poverty?}
The Masaka article discusses the destruction of the city in the 1980's during a civil war and also lists the most common economic activities of its citizens. These types of facts are likely strongly correlated with the regions' economic well-being, but the data is stored as unstructured text. At the same time, many articles (e.g., about historical events) contain information that is likely not relevant for our predictive task --- this makes extracting the relevant information an even more difficult task. 
%harnessing it for analytical purposes an even more difficult task.

An additional challenge is posed by the biased and censored nature of our Wikipedia corpus. The spatial distribution of articles, their length, and their content vary widely across countries and even across regions within the same country. The fact that there are no articles on hospitals in a region obviously does not mean there is no hospital in that region. Similarly, even if an article is present, it might or might not mention aspects that would be useful for our task. Unfortunately, even the probability that relevant facts (e.g., hospital presence) are mentioned in Wikipedia appears to vary significantly across regions. This makes statistical inference much more difficult. This challenge is of course shared by many other sources of social media data, e.g., Twitter messages. However, it does not arise when using a data source such as nightlights, which are collected uniformly and consistently\footnote{Bias due to geography is corrected for using physics-based models.} across the globe.
%While we do not attempt to explicitly model the bias, we found that our models are effective at leveraging the information contained in the Wikiepdia corpus.

Following the proposed framework 
%of using textual-only and multi-modal architectures (text plus nightlights)
, we seek to address the following questions: 
(1) Can we leverage the information in geolocated Wikipedia articles to predict economic indicators, despite the unstructured nature of free text and the inherent bias in the corpus?
(2) How does the quality of the predictions compare to conventional approaches based on remote sensing data?
%(1) Can we demonstrate the same predictive capabilities shown in \cite{Jean790}, extended towards textual representations extracted from Wikipedia articles? 
(3) Is the information from Wikipedia complementary, i.e., can we develop a multi-modal approach utilizing Wikipedia articles  alongside nightlights imagery?
%, to enhance the predictive capabilities of our models? 
%(3) Can textual information lead to a more general model for predicting socioeconomic outcomes across national boundaries? 
%\evan{Is this paragraph necessary/beneficial?}
%\neal{Are these really the questions that we are answering? E.g., for (1) I'm not sure what extending towards textual representations means. It seems like (1) should really be something like, can we use textual representations from Wikipedia articles to make predictions of similar quality (thus paving the way for more general...) For (2), do we really care about enhancing the nightlights-only model, or do we want to know if adding nightlights can enhance our Wikipedia-based approach?}\burak{I agree with Neal that the first question is not clear. To me, it should be proposed as adding textual information improves nighlight only model, not the other way around. Looking at the table 1, NL model is better than Textual only model most of the time. }

%(1)Since the nightlights dataset has been shown to have predictive capabilities, can we demonstrate the same for the textual representations extracted from Wikipedia articles? 
% (2) Does the use of the Wikipedia articles, in combination with nightlights imagery, boost the predictive power of nightlights-only model (i.e. are the two different modalities disjoint such that they represent different features for poverty prediction)? 
% Does the multimodal approach of utilizing Wikipedia articles alongside nightlights imagery, enhance the predictive capability of the nightlights-only model? 


%%%%%%%%%

\subsection{Learning Representations of Wikipedia Articles}
%\evan{Consider changing this title to "Textual Embedding Model" or "Learning Representations of Wikipedia Articles", or something a bit clearer.}

%\s{first thing is to explain the doc2vec part. how to go from text to vectors}
%\s{then new subsection on how to combine multiple article/docs. the averaging stuff}
%\s{then multimodal architecture}
% \subsubsection{Training \textit{Doc2Vec}}
The problem of learning suitable representations for unstructured text data has received increasing attention recently \cite{pang2016text,wang2019learning,lei2015predicting}. 
%cut from here
%\cite{lei2015predicting} perform zero-shot learning using textual descriptors extracted from Wikipedia articles. The textual branch of their multi-modal network predicts the weights of a CNN, allowing them to build one-vs-all classifiers for zero-shot classes at test time. They represent the Wikipedia articles with TF-IDF features that are composed of two terms:(1) Term Frequency and (2) Inverse Document Frequency. The first term measures how frequently a specific term is mentioned while the latter measures the importance of the term.
%Bag-of-Words (BOW) is another method to learn fixed-length feature representations of unstructured text. This method represents a text in terms of a ``bag of words'' by storing the number of occurrences of a word. TF-IDF and BOW representations ignore the ordering of the words and do not project semantically similar words such as ``Power'', and ``Strong'' to a similar space. \neal{I'm not that familiar with these methods but aren't they for representing documents, not words? Why would they be used to project individual words into some feature space?} \burak{Yes they work on documents. You can consider a document with many repetition of "power" and another one with "strong" word. BOW and TF-IDF will not project these two documents to a similar space.}
%BOW can be extended to N-gram models, which store occurrences of phrases of length N instead of words, to somewhat embed word order. \s{cut this whole td-idf section}\burak{If we cut this paragraph, the next paragraph will be meaningless.}
%However, many common methods, such as TF-IDF and Bag-of-Words, struggle to capture long-range semantic dependencies between words. One proposed improvement over these approaches is \textit{Word2Vec} \cite{mikolov2013distributed}, which learns continuous vector representations of words and projects semantically similar words to similar spaces. The model learns continuous vector representations 
%\neal{Is this the right terminology? Maybe ``continuous vector representations''?}
Yet many common methods, such as TF-IDF, Bag-of-Words, and \textit{Word2Vec} \cite{mikolov2013distributed}, struggle to capture long-range semantic dependencies between words.
%--- these models are not suitable here, as they cannot process the semantics of Wikipedia articles. 
The \textit{Doc2Vec} approach~\cite{le2014distributed} remedies these shortcomings by learning robust representations of not only words, but also paragraphs and documents.  \textit{Doc2Vec} captures long-range word dependencies, word orderings, and holistic semantics of words in a document, and has been used in recent studies \cite{wu2018image,ramisa2018breakingnews} that leverage both textual and visual data. Additionally, it has been used on Wikipedia articles to assess the quality of articles \cite{dang2016quality,dang2017end}, with an in-depth empirical analysis presented in~\cite{lau2016empirical}. 
Similarly to these works, we use \textit{Doc2Vec} to embed a Wikipedia article, $D_{i}$, into a $p$-dimensional distributed representation suitable for our downstream task. 
%\matthew{If we need space we can move hyper-parameters to supplementary work.}

To train \textit{Doc2Vec}, we preprocess the body of 1.02 million geolocated Wikipedia articles, $D$, by tokenizing and lowercasing text and removing extraneous punctuation.  This corpus of articles is then fed into a \textit{Doc2Vec} model that utilizes the Paragraph Vector - Distributed Bag of Words (PV-DBOW) training method \cite{le2014distributed} at the suggestion of \cite{lau2016empirical} and others. The model then learns to project the articles to $p$-dimensional vector representations. For this task, we choose a window size of 8, a dimensionality $p$ of 300, and train the model for 10 epochs --- these hyperparameters are similar to those suggested by~\cite{lau2016empirical} as being optimal for similar tasks. We denote the function that is parametrized by the $\textit{Doc2Vec}$ model and returns the $p$-dimensional representation for article $D_i$:
\begin{equation}
    \dembi = \dvec(D_{i}).
\end{equation}
%\evan{The term on the left, $z_{i}^{t}$, needs to be changed, since we define $z_{i}^{t}$ in the wikipedia embedding model section too for something else. Maybe we should use $z_{i}^{a}$? We never explicitly reference the term again anyway.}


 

%\matthew{I think we should put the PCA here}
% The model builds a vocabulary across all documents such that any word which appears in $D$ at least 15 times is included in the vocabulary, denoted $V$. For each article in $D$, \textit{Doc2Vec} randomly initializes a vector with dimensionality $\mathbb{R}^{\alpha}$ and stacks them to form a matrix $P \in \mathbb{R}^{|D| x \alpha}$. 
% \s{unless there is something specific to wikipedia/different from standard doc2vec, this part can be cut. equations confuse people, so avoid them if not striclty necessary. e.g., if you never refer to an equation in the text, you can usually remove it} 

% For each article vector $P_i$, at each iteration $k$, words from the corresponding article $D_{i}$ are randomly sampled to act as the ground truth, and the model utilizes a fully connected layer to make a multiclass prediction over the $k$ randomly sampled words out of the $|V|$ words in the vocabulary. The objective of this model is to maximize the average log likelihood of each random sample $s_1$, $s_2$, ..., $s_T$ of $k$ words, given $P_i$:
% \begin{equation}
%     \frac{1}{T}\sum_{t = 1}^{T}\sum_{j=1}^{k} \text{log } p(s_{t}^{j} | P_i)
% \end{equation}

% This is done using a multiclass classifier, typically a softmax, which is structured as
% \begin{equation}
%     p(s_{t}^{j} | P_i) = \frac{e^{\hat{s}_{t}^{j}}}{\sum_{q=1}^{|V|} e^{\hat{s}_{t}^{q}}}
% \end{equation}
% where $\hat{s}_{t}$ is the prediction vector from the matrix multiplication of the hidden layer's weights $H$ and bias $b$ with $P_i$ 
% \begin{equation}
%   \hat{s}_{t} = P_i^TH + b.
% \end{equation}
% %\neal{Denominator missing}
% The loss is then backpropagated into $P_i$, but not $H$ or $b$, allowing $P_i$ to begin to reflect the holistic semantics of $D_{i}$. Finally, after training the model, we have projected all articles $D_{i}$ to $\alpha$-dimensional representations, $P_i$, using the $i$th column of matrix P as
% \begin{equation}
%     P_i = f_{t}^{1}(D_{i})
% \end{equation}
% where $f_{t}^{1}$ is a function parameterized by the paragraph matrix, $P$.
% \neal{Not sure that this makes sense. Isn't the $\alpha$-dimensional representation of each document stored directly in the paragraph matrix $P$ (also as the rows, not the columns)? Why do we need this function $f_t^1$ and what does the $1$ stand for? How/when do $H$ and $b$ get initialized/updated?}\burak{1 stands for the core function - doc2vec model. 2 stands for the dense layers right before concatenation layer. It is columns. You learn a unique column for each paragraph. Actually, like Evan said, we can just say that $z_{i}^{t}=P_{i}(D_{i})$ or $z_{i}^{t}=f_{t}^{1}(D_{i})$} For training the model, we choose $k$ = 8, $\alpha$ = 300, and train the model for 10 epochs --- these hyperparameters are similar to those suggested by \cite{lau2016empirical} as being optimal for similar tasks.


%\evan{I don't see the point of passing $P_i$ into $f_{t}^{1}$, since $P_i$ is literally the embedded value that the function should be returning anyway. Essentially, $z_{i}^{t}$ will be $P_i$, from what I understand. In my opinion we should just use $z_{i}^{t} = f_{t}^{1}(D_{i})$, say that $f_{t}^{1}$ is parametrized by $P$, and say that in our case $f_{t}^{1}$ is equivalent to passing $D_i$ through the doc2vec, which returns $P_i$. This preserves the generality of $f_{t}^{1}$. This issue carries into the next section too.}

% For this task, we are more interested in the effectiveness of the model in predicting across national boundaries. This guarantees that there is minimal (if any) contamination between train and test data and is more in keeping with traditional benchmarks. 
% \chenlin {Shall we mention 'contamination' here? If so, will people be unconvinced about our later in-country results? It seems like a contradiction if we say contamination here, and we argue that there is no contamination in our results. But we do not want to say there is contamination in our results}

\subsection{Wikipedia Embedding Model}
 
We first propose a model to estimate AWI poverty scores $y_i$ utilizing only textual information in Wikipedia articles in a neighborhood of $\mathbf{c}_i$. 
%This model verifies if there are indeed useful features in the embeddings for poverty prediction.
Suppose that, for a specific country, we have $M$ points where we have DHS ground survey data. 
%At each of these points, we have a location $\mathbf{c}_i = (c_i^{lat}, c_i^{long})$ where $i\in \{1,...,M\}$ and a corresponding wealth index $y_i \in \mathbb{R}$. 
Each of these points corresponds to a location $\loci = (c_i^{lat}, c_i^{long})$ where $i\in \{1,...,M\}$. 
For each $\loci$  we iterate through all the geolocated Wikipedia articles and find $N$ Wikipedia articles 
%$D_{j(1)},...,D_{j(N)}$
$D_{i}^1,...,D_{i}^N$
, each with corresponding location %$((l_{j(1)}^x, l_{j(1)}^y), ..., (l_{j(N)}^x, l_{j(N)}^y))$
$(\mathbf{l}_i^1, \cdots, \mathbf{l}_i^N)$
, 
%\neal{There shouldn't be equals here right?},
that are closest to $\mathbf{c}_{i}$ w.r.t. Euclidean distance.
%,
%\begin{equation}
%d(c_{i},l_{\gamma})=\sqrt{(c_{i}^{x} - l_{\gamma}^{x})^{2} + (c_{i}^{y} - l_{\gamma}^{y})^{2}}.
%\end{equation}
%$j(\cdot)$ stores the indices in $D$ of these $N$ articles, sorted w.r.t Euclidean distance to $c_{i}$. 
We concatenate the $N$ closest article embeddings $(\dvec(D_i^1), \cdots, \dvec(D_i^N))$, each of which is a vector in $\mathbb{R}^{300}$.
Additionally, we compute their Euclidean distances (km) to $\loci$, $(\| \mathbf{l}_i^1-\loci\|,\cdots,\|\mathbf{l}_i^N-\loci\|)$, and use it as an additional feature. This is to capture the potential lack of articles nearby and allow the model to adjust the predictions as necessary.
%\s{adding distance is important to capture lack of articles nearby}
 Thus, the final proposed text embedding can be formulated as:
% \begin{equation}
% z_{i}^{t} = 
% (\dvec(D_i^1), \cdots, \dvec(D_i^N))
% \label{eq:doc2vec}
% \end{equation}
% \begin{equation}
% z_{i}^{d} = (\| \mathbf{l}_i^1-\loci\|,\cdots,\|\mathbf{l}_i^N-\loci\|) 
% \label{eq:dist}
% \end{equation}
\begin{align}
z_{i}^{t} = 
(\dvec(D_i^1), \cdots, \dvec(D_i^N), \|\mathbf{l}_i^1-\loci\|,\cdots,\|\mathbf{l}_i^N-\loci\|) 
\label{eq:dist}
\end{align}
This provides us with a vector in $\mathbb{R}^{300\times N + N}$ \
%as an input feature 
for each $\loci$.
% \begin{equation}
%       z_{i}^{t} = [f_{t}^{1}(D_{j(1)}), f_{t}^{1}(D_{j(2)}), ...,  f_{t}^{1}(D_{j(N)})] 
% \end{equation}
% \begin{equation}
%       z_{i}^{d} = [d(c_i, l_{j(1)}), d(c_i, l_{j(2)}), ...,  d(c_i, l_{j(N)})]. 
% \end{equation}.
%\neal{$z_i^t$ is used earlier to represent the embedding for a single Wikipedia article, now it is being used to represent the concatenated vector of Wikipedia article embeddings for one DHS location. Why can't you just represent each Wikipedia article as the corresponding row of $P$?} \matthew{Is this mathematical representation necessary?}
%\neal{It feels like there are a lot of unanswered questions about this choice of $N$, from very basic ones --- how do you choose it --- to more subtle questions, e.g., does this mean that in places with very sparse Wikipedia articles you are using information from much farther away? Why do it this way instead of aggregating documents within a certain radius, i.e., why choose a different strategy with text data than you would use with image data? Probably would be helpful to discuss this in more detail!}
%\burak{N is experimental. As far as I know, Evan has a figure showing performance vs number of articles considered and the results are better when using 10 articles. Also, we are concatenating feature vectors from N closest articles which does not fit to variable number of articles concept. Besides, we are also providing the distance of an article to the ground truth (See Fig.3 and we should actually mention it in figure 3 caption.)}
%Let $d(p,q)$ denote the Euclidean distance between $p$ and $q$:
%\matthew{I know we did some experiments where we got articles within a fixed radius (10km) but we got better results adding the distance to each article as a feature. My intuition is that the model learns to value features more or less based on the distance  }
%\begin{equation}
%d(p,q)=\sqrt{(p_1 - q_1)^{2} + (p_2 - q_2)^{2}}
%\end{equation}
%\begin{equation}
%      d(y, c) = \sqrt{(y_{x} - c_{x})^{2} + (y_{y} - c_{y})^{2}}
%\end{equation}
%\neal{We should say clearly what $y_i$ are here. The subscripts are confusing right now and $y$ is used several times in different ways.} 
%\chenlin{Take a look at it now, should be fixed}
%with total dimensionality $\mathbb{R}^{300\times N+N}$.
%\neal{This repeats some of the information at the top of the page.}
The combination of textual and distance embeddings are then passed through a neural network consisting of a 3 layer Multi-Layer Perceptron (MLP) with sigmoid and ReLU activations. 
% The final activation is:
% \begin{equation}
%       z_{i}^{w} = f_{t}^{2}([z_{i}^{t}, z_{i}^{d}]).
%       \label{eq:wikipedia_embedding}
% \end{equation}
Lastly
%, given the final embeddings $z_{i}^{w}$, 
we perform regression to predict DHS values (e.g., wealth) for the ground truth point $\loci$.
% \begin{equation}
%     \hat{y} = f_{w}(z_{i}^{w}).
% \end{equation}
A schematic representation of the model is shown in Fig.~\ref{fig:wikipedia_only_model}. 

We empirically determine $N$ (the number of closest articles we consider) in our results section (see Fig.~\ref{Article Iteration Graph}). Fig.~\ref{Article Distances} displays the distances to the closest and 10th closest articles for each wealth coordinate $\mathbf{c}_{i}$. Based on these figures, we find that majority of the articles are within 100 km of their corresponding data point.

%\david{shouldn't this be fig 5 and not fig 9?}


\input{00_article_distances.tex}

% \neal{People can probably make a guess that you chose $N=10$ because of this Figure but you should just say ``We empirically choose $N=10$ (see Fig...)''}\burak{Is it not what we are saying in the sentence starting with ``We empirically". Maybe this is an old comment.}

%We also tried setting a fixed radius neighborhood surrounding $c_{i}$ and averaging the articles' embeddings in the circle, however, our experiments indicate that this averaging operation performs worse. We hypothesize that averaging the embeddings introduces more noise and prevents the model from choosing which articles are more important. 
% For instance, averaging an article related to \emph{hospital} and \emph{celebrity} in a neighborhood reduces the contribution of the \emph{hospital} article which can contain useful information about economic development.  On the other hand, concatenating the Wikipedia embeddings and including the distance allows the model to decide which article embeddings are more important.
%\s{if we need space, this paragraph can be cut}


%%%%%%%%%

%\subsection{Nightlights Only Model}

%\textit{Evan Comment - Not sure this part is necessary}

%\textit{Burak - We can briefly describe it to make the readers familiar with it}
%Recently, \cite{Jean790} proposed a machine learning approach to perform poverty predictions using remote sensing data. Their approach performs transfer learning on Imagenet pre-trained model to learn nightlight features to directly regress poverty scores. By exploring high correlation between nightlight intensities and poverty indexes, they can outperform Imagenet pre-trained model as well as human-conducted surveys using the data collected on the field. Thus, we believe that nighlights information can be highly complementary to information from other modalities to tackle poverty prediction task. Following this strategy, in the next section, we propose a multi-modal architecture that can utilize nighlights and textual information to improve poverty prediction accuracy.

% Recently, \cite{Jean790} showed that the there exists high correlation between nightlight intensities and poverty indices. \s{there's also other prior work in economics that uses nighlights, might want to add a few reference}
% Inspired by this, we take the (5km $\times$ 5km) VIIRS nightlight image centered at $(c_i^x,c_i^y)$ for each point $c_i$, parameterize it by a convolutional deep network, and then pass it through a nonlinear function consisting of a 3 layer Multi-Layer Perceptron (MLP) with ReLU activations which outputs a value indicating the poverty prediction for $c_{i}$. We utilize Mean Squared Error to train the model and iteratively track the $r^2$ of the model (see the Nightlight branch in Figure \ref{fig:workflow}). However, this model is quite limited, especially for countries which have a large portion of the night-time imagery completely dark. To cope with this limitation, we introduce the multi-modal architecture that leverages textual and nightlights data.
% \evan{It's a little strange we don't go into the depth/mathematical notation for this part like we did for the Wikipedia only part. Does it seem fine, and we can just do more signposting saying the notational details are in the multi-modal section?}
% \neal{I think the first part of the multi-modal architecture section should go here if we want to keep this order. Are we worried that if we do that the multi-modal architecture will not seem as novel? If that is the concern, one option would be to switch the order of the sections and present the nightlights-only model as more of an ablation-type thing than as a preliminary/baseline.}
% \s{i like neal's idea of presenting the nightlights only model as ablation. then this section is entirely on novel things, which is less confusing to readers}

%%%%%%%%%

\subsection{Multi-Modal Architecture}
Following our textual only model, we propose a novel multi-modal joint architecture that utilizes nightlight imagery and textual information from Wikipedia. 
%to capture poverty specific features as shown in Fig.~\ref{fig:workflow}. 
%In particular, we want to understand if the textual descriptors can be complementary to nightlights features. 
For each point $\loci$, we utilize our Wikipedia article 
features from Eq.~\ref{eq:dist} as in the previous section. 
%activation features $z_{i}^{w}$ as shown in Eq.~\ref{eq:wikipedia_embedding}.
At the same time, we obtain the (5 km $\times$ 5 km) VIIRS nightlight image $x_{i}$ centered at $\loci$. We then pass $x_{i}$ through a convolutional architecture, the embedding space of which can be represented as $
      z_{i}^{c} = f^{CNN}(x_{i})
$, 
where $f^{CNN}$ is parameterized by a deep convolutional network as shown in Fig.~\ref{fig:workflow} and returns $z_{i}^{c} \in \mathbb{R}^{512}$. We then pass $z_{i}^{c}$ through a nonlinear function consisting of two dense layers with ReLU activations obtaining a vector in $\mathbb{R}^{256}$. 
% \begin{equation}
%     z_{i}^{v} = f_{v}^{2}(z_{i}^{c}).
% \end{equation}
%We perform this step to match the dimensions of two branch before concatenation layer. 
% \neal{I still don't understand why this dense network is considered helpful for rescaling?}\burak{I think they are trying to say that matching the vector dimensions before concatenation is helpful to balance contribution of different modalities, however we do not have any result to support this argument. Maybe we can just say that we run this dense layers to match feature dimensions without saying "it is helpful".}
%\neal{Why should we think of this as a tensor (isn't it a vector) and why do we need to run it through another DNN when we already have a feature vector from the CNN? Maybe the current description isn't clear, but possibly we can also simplify what we're doing --- potential advantages here include being easier to use/implement and also easier to explain.}
%\burak{Do you mean why do we have FC layers after combining feature vectors from two modalities? I did not understand what you mean by "running it through another DNN".}
Next, we concatenate representations from the two different modalities 
%in the following way:
% \begin{equation}
%     z_{i} = [z_{i}^{v}, z_{i}^{w}].
% \end{equation}
% Finally, the multi-modal representation $z_{i}$ is forwarded to another nonlinear function, $f_{c}$, with \david{could be more precise on number of layers/activations} 
and use another 
four dense layers, each with a ReLU activation, and a final regression layer to produce the final estimate.
%predicted wealth level:
% \begin{equation}
%     \hat{y}_{i} = f_{m}(f_{c}(z_{i})).
% \end{equation}
The proposed architecture, as shown in Fig.~\ref{fig:workflow}, is jointly trained on the task of poverty prediction. However, we freeze the weights of the $Doc2Vec$ during training on the poverty task.

%%%%%%%%%

\input{00_workflow.tex}



% \begin{figure*}[h]
%     \begin{subfigure}{.5\textwidth}
%         \centering
%         \includegraphics[width=3.1in]{diagram/wiki_pearson.png}
%     \end{subfigure}
%     \begin{subfigure}{.5\textwidth}
%         \includegraphics[width=3.2in]{diagram/CNN-PearsonR.png}
%     \end{subfigure}
%     \caption{\textbf{Left:} Pearson's r squared values obtained for models trained on the embeddings of the column countries and tested on the embeddings of the row countries. \textbf{Right:} Pearson's r squared values obtained for models trained on the embeddings + Nightlights of the column countries and tested on the embeddings + Nightlights of the row countries.}
%     \label{FCL Model}
% \end{figure*}

% \begin{center}

==> Poverty Prediction using Remote Sensing Data andText Information(KDD) Arxiv Copy/0_related.tex <==
% \section{Related Work}
% %\s{move related work at the end}
% Representation learning has been used in a variety of tasks to distill high dimensional data to a latent space representation. \cite{stewart2017label}
% %Neal: Is this citation relevant?
% This has manifested itself in recent advancements which have created models to learn representations for satellite imagery \cite{jean2018tile2vec} and text corpora \cite{miller1995wordnet}. In our work, we use \cite{le2014distributed} to learn a latent space representation for Wikipedia articles. This approach is validated by \cite{lau2016empirical}, who also train a Doc2Vec model on the English Wikipedia corpus and specify optimal hyperparameters for the task. Deep learning has been applied to satellite imagery in the context of structure classification \cite{xia2018dota}, map segmentation \cite{wang2015deep} \cite{audebert2017joint}, and pattern identification \cite{albert2017using}. Previous work has explored predicting humanitarian indicators using satellite imagery. \cite{kim2006satellite} uses satellite imagery to predict $NO_x$ emissions, and \cite{pinkovskiy2016lights} \cite{Xie2016TransferLF}\cite{wang2012poverty} \cite{nips_2017_workshop_stefano} utilize Nightlight to predict poverty, while \cite{Jean790} also use RGB satellite imagery and transfer learning. with promising results. \cite{henderson2012measuring} and \cite{pinkovskiy2016lights} \cite{Xie2016TransferLF} also utilize features derived from satellite imagery to extract features for poverty prediction. 
% \evan{We should figure out how to balance the paragraph in the intro about social media and socioeconomics with this section.}

%%%%%%%%%


==> Poverty Prediction using Remote Sensing Data andText Information(KDD) Arxiv Copy/0_results_education.tex <==
\section{Education Index Prediction}

%Eliminating poverty may be the first of the UN SDGs, but true progress towards global sustainability will require advances on multiple fronts. As with poverty, measuring progress on these other goals will be possible only with quality data --- multi-faceted and general approaches based on datasets that contain signal about multiple socioeconomic indicators are more valuable than those that can only be used for a single purpose.

To further test the effectiveness of our text-only model in predicting other socioeconomic outcomes, we train and evaluate our model on a new task: education level-prediction.
Improving the quality of global education is the 4th SDG --- access to education is foundational to the creation of self-sustaining and self-improving societies.

In addition to predicting a different type of outcome, we use a new source of ground truth data for this task. We use the Afrobarometer R6 Codebook dataset \cite{AFRO}, which is distributed by Afrobarometer, a research network that conducts public attitude surveys on democracy, governance, economic conditions, and related issues in more than 35 countries in Africa. We utilize the `eaeducationlevel' index, which has values ranging from 1 to 4, with larger number standing for higher level of education (i.e., 1 stands for `No formal schooling', 4 stands for `post-secondary qualifications'), for our groundtruth labels. To be consistent with the previous experiments on poverty, we limit our research to 5 countries (see Table \ref{table:Education Results Table}) in Africa, each with 300 datapoints. Notice that Afrobarometer is sampled at different locations compared to DHS.
%we re-collect the N=10 closest Wikipedia articles embeddings together with the distance, and concatenate them into an input vector in $\mathbb{R}^{300\times N+N}$. 
We evaluate our Wikipedia Embedding model on the (a) Intra-nation and (b) Cross-Boundary training tasks, as in the previous section. We use the same training procedure, except we regress on a different outcome.

Table \ref{table:Education Results Table} displays our results on this task. We notice that that in-country models (shaded) consistently outperform out-of-country models, as was generally the case for the poverty task. However, on average the performance is worse compared to the poverty task, with averages ranging from .20-.25 compared to .40-.45. One possible explanation is that education is a finer-grained indicator that is more difficult to predict from Wikipedia. We can expect improved results with the inclusion of more education-related articles in future releases.
%\s{maybe say not many elementary schools in wikipedia? is that true?}.
Nevertheless, this experiment suggests that Wikipedia provides useful information to predict multiple socioeconomic indicators, across different countries and even different survey methodologies.

%% can we add an average column to the table?


%\burak{Is there a reference for this dataset} \matthew{add dataset citation here}

\input{00_table_education.tex}

==> Poverty Prediction using Remote Sensing Data andText Information(KDD) Arxiv Copy/0_results_poverty.tex <==
\section{Poverty Prediction}

\input{00_table_poverty.tex}

Our study proposes novel single and multi-modal deep neural networks that predict economic development using a combination of Wikipedia and remotely sensed data (nightlights). To compare with prior work and put our results into perspective, we also consider a baseline \nightonly{} model,
which only uses nightlights as an input. Our \nightonly{} model is based on the ``nightlights branch" of the proposed multi-modal architecture in Fig.~\ref{fig:workflow}. This allows us to directly evaluate the contribution of Wikipedia articles in the multi-modal model. We emphasize that this is a strong baseline model, as previous works use simpler, hand-crafted features, such as the mean intensity or simple summary statistics (max, min, median), instead of the image \cite{noor2008using}. Such simpler nightlight models are not included in this study as they significantly underperform our CNN-based \nightonly{}  model. We additionally compare to a model from~\cite{Jean790} that uses a combination of nighlights and high-resolution satellite images.

All the architectures are evaluated on three experiments:
\begin{itemize}
    \item [(a)] Intra-nation tests: Train and test on the same country.
    \label{intra}
    \item [(b)] Cross-national boundary testing between African countries: Train on one country and test on another.
    \item [(c)] Leave-one-country-out training: Train on all countries except one and test on that country, and vice versa. 
\end{itemize}
These experiments were chosen as they reflect the possible real-world applications of this model. 
In particular, (a) intra-nation inference can be used to fill in gaps of surveys within a country. Data acquired using this method can be very useful in providing local government with the tools to efficiently target aid. 
Cross-national boundary (b) and leave-one-out based predictions (c), on the other hand, can be used to make predictions in countries with no recent survey data. 
%These can be areas where civil and political unrest is occurring, or areas where on-the-ground collection is impossible. 

As we regress directly on the poverty index, we measure the accuracy of our model using the square of the Pearson correlation coefficient (Pearson's $r^2$). 
%The Pearson correlation coefficient measures the linear correlation between two variables $x$, $y$ (in this case the ground truth and predicted value).  
%An output value of $1$ corresponds to perfect linear correlation whereas $0$ stands for no correlation. 
%The square of the Pearson correlation coefficient, on the other hand, represents the proportion of variance in $y$ explained by a linear function of $x$. 
% \begin{equation}
%     r_{s_{i}, y_{i}}^{2} = \Bigg( \frac{\sum_{i=1}^{M}(\hat{y}_{i}-\bar{\hat{y}})(y_{i}-\bar{y})}
%     {\sqrt{\sum_{i=1}^{M}(\hat{y}_{i}-\bar{\hat{y}})^2}
%     \sqrt{\sum_{i=1}^{M}(y_{i}-\bar{y})^2}}
%     \Bigg)^2
% \end{equation}
% where $\hat{y}_{i}$ represents the model prediction at $c_{i}$ and $y_i$ represents the ground truth. 
This metric was chosen so that comparative analysis could be performed with previous literature \cite{Jean790,nips_2017_workshop_stefano}. Further, in cases of out-of-distribution testing, such as cross-national boundary tests, linear correlation can still be a meaningful metric. For example, our model may have slightly lower predictions if it is trained on a relatively poor country and tested on a wealthy one.
%, as it has never seen high wealth indices during training. 
In this case, comparing the absolute predicted value with the ground truth would not be a fair option. On the other hand, Pearson's $r^2$ is invariant under separate changes in location and scale between the two variables. This allows the metric to still provide insight into the ability of the model to distinguish between poverty levels. In the space of aid, knowing relative wealth indices is often a good alternative to knowing the true ground truth values, as it still provides insight on where to target aid. 

%%%%%%%%%

\subsection{Wikipedia Embedding Model}

We train our \wikipedia{} (WE) model using a Mean Squared Error loss function, along with an Adam optimizer with a learning rate of 0.001. We report in Table \ref{table:Results Table} $r^2$ values obtained from  (a) intra-nation (shaded in blue), as well as (b) cross-country  and (c) leave-one-out evaluations. 

\textbf{In-Country:} We observe that our \wikipedia{} (WE) model is able to robustly learn associations with poverty. Compared with the \nightonly{} (NL) model, we see that WE outperforms NL in all 5 countries. Comparing to the state of the art results from~\cite{Jean790}, which are based on a combination of nighlights and high-resolution daytime imagery, we see that we are consistently within $10$-$15\%$ of the reported $r^2$'s for training and testing on the same countries, except for Tanzania, where we improve from .58 to .64. 

\textbf{Out-of-Country:} 
Cross national boundary experiments allow us to test the generalization capabilities of the model. As we are taking 5 km $\times$ 5 km nightlight images of a data point, there may be portions of images similar to both train and test sets because of underlying spatial correlations between the examples. This can also happen for the Wikipedia embeddings, as the $N$ = $10$ closest articles can have some overlap between training and testing examples when evaluating within the same country. Prediction across national boundaries is a more difficult task, both because of covariate shift and because there is almost no spatial correlation between the train and test sets the model can exploit. 

The details of these results are in Table~\ref{table:Results Table}, where the statistics of a model trained on country A and evaluated on country B are located in the column labelled A and the row labelled B. 
%This column A contains 3 subcolumns, representing from left to right the Nightlights-Only Model's results (NL), the Wikipedia Embedding Model's results (WE), and the Multi-Modal Model's results (MM) when that specific model, trained on A, was evaluated on B. 
The ``Average'' row simply presents the average performance of the 
%NL, WE, and MM (Multi-Model; see next section for detailed MM results) 
models for each column country.
%\neal{I still think it's kind of weird to have an average row, also we refer to MM model here before introducing MM.}
For example, Fig.~\ref{Combined Raster} displays the results of the WE model when it is trained on the Ghanaian article distribution and then evaluated on the Tanzanian article distribution. We observe that, while the model may not always predict the correct wealth level for a region, it is often correct in its \emph{relative} predictions for adjacent regions and regions within the nation in general. This suggests that scaling the model by the mean income level for a country (data which is available) may allow the model to correctly determine both relative and absolute wealth levels.

%PLOT 
\begin{figure}[h!]
    \centering
    \includegraphics[width=3.5in]{GHA_TZA_groundtruth_predicted_.png}
    \caption{\textbf{Left:} Ground truth values of 1074 data points averaged on Admin 2 Level for Tanzania. \textbf{Right:} Wikipedia Embedding Model predicted values averaged on Admin 2 level for a model trained on Ghana and tested on Tanzania ($r^2=0.52$). The resulting predictions show that the model is capable of generalizing across national boundaries.}
    \label{Combined Raster}
\end{figure}

Comparing WE to NL for out-of-country experiments, we see that NL often outperforms WE by a very slight margin, usually by approximately .1 to .15 in terms of $r^2$. This is also true when comparing WE to the out-of-country state of the art results from \cite{Jean790}. The exception to both these trends is that WE outperforms both NL and \cite{Jean790} by about .05 to .1 on over half the models either trained or tested on Malawi. Throughout all these results, the core theme observed is that the WE model is learning generalizable features and not simply picking up on spatial correlations, since the train and test sets are \emph{entirely} disjoint.

%\s{compare to NL first, then to [12]. explain to the reader how to read the table. tell reader explicitly that it's not just picking up spatial correlations}
%\s{text below and fig explains why WE is better than NL}
%\s{swap fig with one where WE is better than NL}
To better understand the role of Wikipedia embeddings, we 
%perform a case study comparison of a baseline model trained on nightlights imagery only (and having the same architecture as the CNN branch of Fig.~\ref{fig:workflow}) and the WE model. 
visualize the predictions of the NL and WE models trained on Ghana and tested on Tanzania in Fig.~\ref{Prediction}. Because certain countries' nightlights datasets are dominated by dark images, in certain circumstances the \nightonly{} model is prone to predict constant values, which results in the horizontal line of predictions shown in the left plot of Fig.~\ref{Prediction}. However, the \wikipedia{} model does not suffer from such a shortcoming and is able to increase the range of the predictions, 
%alleviating the problem of constant prediction 
as shown in the right plot of Fig.~\ref{Prediction}.

%Across national boundaries, we observe mixed results. While we do not match the results of \cite{Jean790} for a majority of the cross-national boundary experiments, we achieve promising results, with $r^2$'s of approximately .4-.5 for most countries.

\input{00_nl_we.tex}

\textbf{Leave-One-Out:} 
%\s{the africa thing is never explained. based on the table, it seems that we can say that on average, it's better to train on africa (0.49) than any single country, but for some pairs it's better to use data from a single country, e.g. africa-ghana vs tanzania-ghana. this makes sense because we might want to weight more data from similar countries.}
The column ``All'' in Table~\ref{table:Results Table} represents models trained using the leave-one-out approach, such that a model in column ``All'' evaluated on nation $B$ was trained on all countries but $B$.
%the set of countries 
%$\{$Ghana, Malawi, Nigeria, Tanzania, Uganda$\}$ - $\{$B$\}$.
The inverse is true for row ``All'', where a model trained on nation A is
tested on all other countries.
%$\{$Ghana, Malawi, Nigeria, Tanzania, Uganda$\}$ - $\{$A$\}$.

Examining the leave-one-out experiments, we observe that training with this approach achieves the best results on average compared to training on any other single country. The average $r^2$ of WE models trained in this way is .49, the highest such WE model averages. Interestingly, the models trained on only Tanzania perform similarly or even better than the ones trained on All countries on the Malawi test samples. We hypothesize this is due to similar patterns of the neighboring countries in the dataset.


% \neal{Ah ok I see, the stuff in the previous paragraph is a little more clear now. Maybe we should explain this train-test split danger earlier and in one place.} 
% The results of the "leave one out" approach of training on Africa (other 4 countries) and testing on one nation on average performs better than on any other single country. However, some country pairs have better cross-country results (Tanzania-Ghana). We hypothesize that this is because the spread of wealth between the two countries is similar or correlated. 

% does not necessarily lead to better results according to the $r^2$ metrics than the cross-boundary models, despite being trained on many times more datapoints. We hypothesize that this is due to the model being trained on a combination of many noisy article distributions from the entire continent, but being evaluated only on one such distribution. 
% %^While the model achieves incredible results when evaluated on a test set from itself 
% \neal{What does this mean? Which results is this referring to?}
% %, this can possibly be attributed to its greater training set size causing higher interpolation between its train and test sets. 
% \matthew{I'm confused with this explanation.. The low overall in Africa could just mean that nightlights in general is a better predictor? and that using Wikipedia is there to help but not necessarily outperform.} \evan{we need to come up with an intuitive explanation for the Africa experiments. we also need to explain the country splits (ie define "Africa")}

%\subsection{Education Index Prediction}
%\input{education}





% \matthew{Are we putting this? If yes, we should put the plots somewhere}
% \burak{This part should be removed.}
% Additionally, to better understand the article embeddings and their significance, we evaluated our models on Uganda, utilizing our Average MLP model, to analyze the 300 dimensional inputs to see which embedding indices were most important for the model's predictions. We did this by evaluating the model 300 times, each time masking all but one of the input dimensions, and observing the resulting $r^2$ values. We found several indices, most notably indices 24 and 182, that were highly predictive (obtaining .3 and .4 $r^2$ by themselves). Searching our inputs, we found that Ugandan articles which possess the highest values at these indices are often those related to healthcare and education (ie. hospitals and schools). This analysis is very informative, as it reveals that  our model is learning to look at the healthcare and education of a region (via Wikipedia articles) in order to predict the poverty of the region. In other words, our model is learning that the healthcare and educational status of a region is very informative for predicting poverty, which, in reality, is true. 
% \evan{Not sure if this should be included. Should probably be moved up with the PCA in methods maybe if so? Also need to think about including egypt and bolivia experiments.}

%%%%%%%%%
%%%%%%%%%

\subsection{Multi-Modal Model}

We train our \multimodal{} (MM) model using a Mean Squared Error loss function, along with an Adam optimizer with a learning rate of 0.001.
Table \ref{table:Results Table} displays the Pearson's $r^2$ results of the model. Comparing WE with MM, we observe that in general the accuracy ($r^2$) of the models 
for out-of-country evaluation 
%trained on specific nations and applied to the other countries 
improves by almost 50\% across the board for the multi-modal approach. Importantly, the proposed multi-modal architecture outperforms the other models by large margin when trained via the leave-one-out approach, proving that the textual branch maintains its contribution even when training the CNN with large amounts of nightlights data. Some models, such as the one trained on Uganda and tested on Nigeria, obtain over $100\%$ improvement, while others, such as the one trained on Ghana and tested on Tanzania, obtain less than a $20\%$ improvement. Importantly, all train-test country combinations see some degree of improvement. When considering the results of our ablative \nightonly{} model, we also observe that the MM achieves superior results for both intra-country and cross-boundary tests nearly across the board. 
%\evan{should we qualify the NGA-GHA and UGA-GHA NL results here briefly?}
Such results suggest that Wikipedia embeddings and nightlight images provide highly complementary information about poverty. Finally, the MM outperforms state of the art by an average of $31.2\%$ \cite{Jean790}, with improvements nearly across the board. 

%Such results seem to point to the fact that the article embeddings and the nightlights imagery contain complementary information and capture different features useful for poverty prediction, allowing them to be utilized together by the network and thus often beating the state-of-the-art results from \cite{Jean790} by $30-40\%$ (see Figure \ref{Improvements} for a detailed comparison with state-of-the-art).
%\neal{Is there a way to assess this directly? Maybe see if you can predict nightlights from articles, estimate mutual information, etc. Feels like a little bit of analysis might go a long way here to placate reviewers.} \evan{we are presenting it like an ablation study I believe now.}


\begin{comment}
\begin{figure*}[h!]
    \begin{subfigure}{.5\textwidth}
        \centering
        \includegraphics[width=3in]{diagram/combined_improvements.png}
    \end{subfigure}
    \begin{subfigure}{.5\textwidth}
        \centering
        \includegraphics[width=2.5in]{diagram/philippine_prediction.png}
    \end{subfigure}
    \caption{\textbf{Left:} Improvements in results from \cite{Jean790}. Our model makes substantial improvements especially in countries with minimal data from nightlights. \textbf{Right: } Example of real-world application where a model trained on Africa is tested on a country with no ground-truth data. Note that the model predicts a range of poverty levels. A cursory analysis showed that it correctly predicts relative wealth between major cities and rural areas.}
    \label{Improvements}
\end{figure*}
\end{comment}
